FedMVP: Federated Multimodal Visual Prompt Tuning for Vision-Language Models

In federated learning, textual prompt tuning adapts Vision-Language Models (e.g., CLIP) by tuning lightweight input tokens (or prompts) on local client data, while keeping network weights frozen. After training, only the prompts are shared by the clients with the central server for aggregation. However, textual prompt tuning suffers from overfitting to known concepts, limiting its generalizability to unseen concepts. To address this limitation, we propose Multimodal Visual Prompt Tuning (FedMVP) that conditions the prompts on multimodal contextual information - derived from the input image and textual attribute features of a class. At the core of FedMVP is a PromptFormer module that synergistically aligns textual and visual features through a cross-attention mechanism. The dynamically generated multimodal visual prompts are then input to the frozen vision encoder of CLIP, and trained with a combination of CLIP similarity loss and a consistency loss. Extensive evaluation on 20 datasets, spanning three generalization settings, demonstrates that FedMVP not only preserves performance on in-distribution classes and domains, but also displays higher generalizability to unseen classes and domains, surpassing state-of-the-art methods by a notable margin of +1.57% - 2.26%. Code is available at https://github.com/mainaksingha01/FedMVP.

==> supple_tables/parameters.tex <==


\begin{table}[t]

    \centering
    \caption{{\textbf{\btoncap setting.}} Accuracies (\%) on client's local (seen) classes, base (seen) classes and new (unseen) classes. Harmonic mean (HM) is computed with Base and New class accuracies. Best number in each column is in bold.}
    \vspace{-.2cm}
    \scalebox{0.69}{
    \begin{tabular}{lcccc|ccc}
    \toprule
        
        \textbf{Methods} & \textbf{Prompts} & {Local} & {Base} & {New} & {HM} & {T. Params}\\ 
        \midrule
         
        ZS-CLIP \cite{clip} &hand-crafted &76.72	&70.51	&75.78	&\cellcolor[gray]{0.9}74.24 & 0 \\ 
        \midrule
        FedOTP \cite{fedotp} &\multirow{4}{*}{textual} &74.82 &65.22 &57.04 &\cellcolor[gray]{0.9}64.89 &16,384 \\
        FedKgCoOp \cite{kgcoop} & &78.38	&72.18	&75.87	&\cellcolor[gray]{0.9}75.39 &2048 \\
        PromptFL \cite{promptfl} & &\textbf{81.75}	&74.47	&71.70	&\cellcolor[gray]{0.9}75.74 &2048 \\
        FedTPG \cite{fedtpg} & &80.75	&73.68	&76.02	&\cellcolor[gray]{0.9}76.70  &4.2M\\
        \midrule
        FedCLIP \cite{fedclip}&visual &76.87 &71.04 &75.06 &\cellcolor[gray]{0.9}74.24 &0.52M  \\
        \midrule
        FedCoCoOp \cite{cocoop}&\multirow{3}{*}{textual+visual} &81.46	&73.76	&66.00	&\cellcolor[gray]{0.9}73.20 &35,360 \\
        
        FedMaPLe \cite{maple}& &81.63	&74.44	&70.62	&\cellcolor[gray]{0.9}75.29 &3.55M\\
         
        \method (Ours) & &80.80	&\textbf{74.50}	&\textbf{77.51}	&\cellcolor[gray]{0.9}\textbf{77.52} &19.3M \\

\bottomrule
    \end{tabular}}
    \label{tab:base2new}
    \vspace{-0.5cm}
\end{table}




